Enhancing Biomedical Text Summarization and Question-Answering: On the Utility of Domain-Specific Pre-Training

Biomedical summarization requires large datasets to train for text generation. We show that while transfer learning offers a viable option for addressing this challenge, an in-domain pre-training does not always offer advantages in a BioASQ summarization task. We identify a suitable model architecture and use it to show a benefit of a general-domain pre-training followed by a task-specific fine-tuning in the context of a BioASQ summarization task, leading to a novel three-step fine-tuning approach that works with only a thousand in-domain examples. Our results indicate that a Large Language Model without domain-specific pre-training can have a significant edge in some domain-specific biomedical text generation tasks.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> sections/1-introduction-v0.tex <==
% !TeX root = ../main.tex
%
\section{Introduction}
%● tasks performed
%● main objectives of experiments

We are looking for solutions for a summarization challenge presented by BioASQ Task B Phase B (text summarization). 
Historically, question-answering and extractive summarization were primarily approached as classification problems. 
Since then, abstractive summarization models have demonstrated much better results and a greater capacity for generalization, effectively blurring the line between long-form question answering and summarization. 
We use term generation tasks to refer to summarization and long-form question answering. 
The generation model needs to produce clear and coherent answers based on the set of inputs (context) provided to the model.

The BioASQ task is performed in the biomedical domain.
Healthcare presents countless opportunities to benefit from health-research data sharing in areas such as clinical care, informed clinical choice, and scientific discovery, to name a few \cite{Krumholz2016}. 
\emph{Pre-trained language models} (PLMs) could be an excellent candidate for sharing bio-medical and healthcare studies and research data with the wider public. 
In the future, PLMs could store medical knowledge while considering differences in data or even in the application tasks \cite{Bommasani2021}.

% This study analyses how a training process affects PLMs abilities to store biomedical knowledge  with an objective of providing guidance for utilising them for question answering and summarization tasks. 
 
The default approach for achieving the best results on natural processing tasks is pre-training models, followed by task-specific fine-tuning \cite{Vaswani2017, Devlin2018}. 
PLMs have re-defined modern approaches in every area of NLP \cite{mikolov13,Peters2018,Devlin2018}. 
Generally speaking, such models are trained on an extensive range of texts and topics and then applied to downstream tasks via fine-tuning on large datasets \cite{Devlin2018,Lewis2019,Bommasani2021}. 
We refer to this as a two-phase training approach (shown in the top row of \cref{figure:tl-diagram}), where the model is pre-trained and then fine-tuned directly on the target task. 
However, pre-training is long and expensive and information on how these models perform for domain-specific applications with limited data availability remains sparse. 
In this work, we study one such application presented by the summarization task of a BioASQ challenge.

Over the last five years, the biomedical domain has grown to rely on in-domain pre-training and (sometimes) fine-tuning BERT \cite{Devlin2018} for a range of in-domain datasets and benchmarks \cite{Alsentzer2019,Lee2019a,Gu2020,Alrowili2021,Raza2022}. 
In-domain pre-training improves results when using BERT for discriminatory biomedical tasks. 
However, BERT \cite{Devlin2018} is not a very effective architecture for text generation tasks.
This is because it does not use an autoregressive decoder, which would allow it to generate tokens based on the previously generated tokens. 
Instead, BERT relies on the entire context, making it a suboptimal choice for generation tasks \cite{Liu2019b, Raffel2019}. 
A notable study that reviewed a range of biomedical models on a diverse selection of tasks has not reported results on generation problems because they have only used non-autoregressive models \cite{Gu2020}. 

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.7\textwidth,height=\textheight,keepaspectratio]{tl-diagram.png}
  \caption{
    \textbf{Schematic representation of PLM usage in practice.}
    The top row represents the two-phase "training then fine-tuning" approach typically deployed in literature.
    The middle and bottom rows represent the task-specific fine-tuning approach proposed in this paper. 
    Our results suggest that in-domain training does not improve the BioASQ summarisation performance even when summarization training is introduced in the middle (second row). 
    In this diagram, the orange area indicates in-domain training.
  }
  \label{figure:tl-diagram}
\end{figure*}

A significant amount of research suggests that domain-specific pre-training significantly outperforms mixed-domain pre-training. 
However, we could not find any convincing evidence for supporting this belief when it comes to text generation problems \cite{Alsentzer2019,Lee2019a,Gu2020,Alrowili2021,Yuan2022,Luo2022,Raza2022}. 
In this work, we observe that having a large task-specific dataset can be more valuable than domain-specific pre-training when fine-tuning for biomedical text generation. 
At first glance, this goes against some of the established theories in the biomedical domain, even when it comes to the generation tasks \cite{Gu2020, Yuan2022, Luo2022}. 
Intuitively, one can achieve higher performance by chaining three steps (shown in the bottom row of \cref{figure:tl-diagram}): first train a general-domain PLM, followed by fine-tuning for a specific task in the general domain (here text summarization), and finally fine-tunning for the target biomedical domain.
in support of our approach, studies suggest that diverse pre-training objectives, larger and more diverse datasets and tasks can increase the robustness of the fine-tuning process even without domain adaptation \cite{Raffel2019, Hendrycks2020}.  
 
 % main contribution
 BART \cite{Lewis2019} can be seen as a generalization BERT \cite{Devlin2018} and GPT \cite{Radford2018} architectures;
 it introduces useful pre-training objectives. 
 This architecture achieves state-of-the-art results on various abstractive dialogue, question-answering, and summarization tasks, particularly effective in text generation and comprehension tasks. 
 This paper evaluates the benefits and effectiveness of using this architecture for applying transfer learning techniques on a biomedical summarization task.
 
 \textbf{The main contributions of this work can be summarized as follows:}

\begin{itemize} 
\item evaluating benefits of domain-specific pre-training in a context of text generation tasks
\item evaluating if task-specific training helps text generation tasks
\item evaluating how (an encoder with an auto-regressive decoder architecture of) BART performs on a (domain-specific) biomedical question answering task B in BioASQ 11
\end{itemize}
